Moving Away from the Joneses to Move Ahead: Migration, Information Gap and Signalling

Signalling social status through the consumption of visible goods has often been perceived as a way in which individuals seek to emulate or move up compared to others within the community. Using representative migration survey data from the Indian state of Kerala, this paper assesses the impact of transnational migration on consumption of visible goods. We utilize the plausibly exogenous variation in migration networks in the neighbourhood and religious communities to account for the potential endogeneity. The findings indicate a significantly positive and robust effect of migration on conspicuous consumption, even after controlling for household income. In terms of the mechanisms, while we are unable to rule out the associated taste-based changes in preferences and the peer group effects driving up the spending on status goods, we observe only limited effects of these channels. A potential channel that we propose is information gap among permanent residents about the income levels of an out-migrant, which is leveraged by them to signal higher status in society. We explore this channel through a theoretical model where we connect migration, information gap and status good consumption. We derive a set of conditions to test whether migrants exhibit snobbish or conformist behaviour. Empirical observations indicate predominance of a snobbish behaviour.

==> jan 2021/AlternativeDepVars.tex <==
\begin{longtable}[t]{l c c c }
	
	
	\caption{Robustness -- Alternative Dependent Variables \label{tab:alt dep}} \\
	%
	
	\hline \hline
	\endfirsthead
	
	\multicolumn{4}{l}%
	{{ \tablename\ \thetable{} -- continued from previous page}} \\
	\hline
	\endhead
	
	\hline
	\multicolumn{4}{r}{{Continued on next page}} \\
	\endfoot	
	
	\endlastfoot
	
	
	
	\multicolumn{4}{c}{{ Dependent Variable:  }}    \\
	\multicolumn{4}{c}{{ {\bf Standardized Visible Consumption Index} }}    \\
	\hline
	International Migrant 	&   0.315*  &               &               \\
Household	&     (0.164)   &               &               \\		
	\\
	Household Ever had  	&             &       0.189** &               \\
International Migrant	&               &     (0.095)   &               \\
	\\	
	Log Remittances	&               &               &       0.028*  \\
	&               &               &     (0.015)   \\	
	
	\hline \hline
	
	\multicolumn{4}{c}{{ Dependent Variable:  }}    \\
	\multicolumn{4}{c}{{ {\bf Conspicuous Consumption Household} }}    \\
	\hline
	International Migrant 		&   0.666** &               &               \\
Household	&     (0.266)   &               &               \\	
	\\
	Household Ever had  	&            &       0.376** &               \\
International Migrant	&               &     (0.160)   &               \\
	\\	
	Log Remittances	&                 &               &       0.060** \\
	&               &               &     (0.024)   \\	
	\hline \hline
	
	
	\multicolumn{4}{c}{{ Dependent Variable: {\bf Luxury House} }}    \\
	\hline  
International Migrant	& 1.068***&               &               \\
	Household&     (0.318)   &               &               \\		
	\\
	Household Ever had  	&              &       0.603***&               \\
International Migrant	&               &     (0.204)   &               \\
	\\	
	Log Remittances	&               &               &       0.096***\\
	&               &               &     (0.028)   \\
	
	\\
	
	F-statistic	&              266.637       &     1159.263 &     218.153  \\
	
	
	\hline \hline
	
	\multicolumn{4}{p{0.60\textwidth}}{\footnotesize Note: Definition of the dependent variables are given in Table \ref{tab:def}. All models control for covariates in Table \ref{tab:fullmodel}. The results reported are of IV models instrumented with migration network at Village level and Taluk-Religion level. Clustered standard errors at the village level are reported in the parentheses. The F-statistic refers to the Wald version of the Kleibergen and Paap rk-statistic. The number of observations is 14,325 in all models. * \(p<0.10\), ** \(p<0.05\), *** \(p<0.01\)}
	
\end{longtable}

==> jan 2021/Plausexog.tex <==
\begin{table}[thb!]
		\caption { Plausibly Exogenous IV Analysis} \label{tab:plausexog} 
		\begin{tabular}{ >{\arraybackslash}p{2 in} >{\arraybackslash}m{1 in} >{\arraybackslash}m{1 in} >{\arraybackslash}m{1 in} >{\arraybackslash}m{1 in}}
			\hline \hline
			& \centering Visible Consumption Index (PCA) & \centering Visible Consumption Index (Stan.) &\centering Conspicuous Consumption Household  & Luxury House \\
			\hline 
			\\
			\centering	OLS	&\centering 0.228***  &\centering 0.192*** &\centering 0.358***  & 0.433*** \\
			&\centering (0.023) &\centering (0.022) &\centering (0.039)  & (0.040) \\
			
			
			\\
			\centering	IV - 2SLS	&\centering 0.408**  &\centering 0.315* &\centering 0.666**  & 1.068*** \\
			&\centering (0.160) &\centering (0.164) &\centering (0.266)  & (0.318) \\
			\\
			\centering	Plausibly Exogeneous		&\centering 0.756*** &\centering 0.698*** &\centering 0.309*** & 0.529*** \\
			
			&\centering (0.160) &\centering (0.165) & \centering (0.077)  &   (0.111) \\
			\\ 
			\centering	Plausibly Exogeneous		&\centering 0.756***  &\centering 0.698*** &\centering 0.309*** & 0.529***  \\
			\centering	(with uncertainity)		&\centering (0.167) &\centering (0.172) &\centering (0.081) & (0.116) \\
			\\
			\hline \hline
			\multicolumn{5}{p{\textwidth}}{\footnotesize Note: The treatment variable is `International Migrant Household'. All models control for covariates in Table \ref{tab:fullmodel}. Clustered standard errors at the village level are reported in the parentheses. The row ‘Plausibly exogenous’ assumes $\Omega_r = 0$ and ‘with uncertainty’ uses $\Omega_r = (0.125 \sqrt{s_i^2 + s_r^2})^2$. * \(p<0.10\), ** \(p<0.05\), *** \(p<0.01\)}
			\end {tabular}
		\end{table}

==> jan 2021/alt.tex <==
\begin{longtable}[thb!]{l c c c }
	
	
	\caption{Alternative Channels - Preferential Changes \label{tab:alt}} \\
	%
	
	\hline \hline
	\endfirsthead
	
	\multicolumn{4}{l}%
	{{ \tablename\ \thetable{} -- continued from previous page}} \\
	\hline
	\endhead
	
	\hline
	\multicolumn{4}{r}{{Continued on next page}} \\
	\endfoot	
	
	\endlastfoot
	
	
	
	\multicolumn{4}{c}{{ Dependent Variable: {\bf Log Food Expenditure } }}    \\
	\hline
	\\
International Migrant&       0.076   &               &               \\
 Household&     (0.140)   &               &               \\
Household Ever had &               &       0.048   &               \\
International Migrant &               &     (0.080)   &               \\
Log Remittances     &               &               &       0.007   \\
&               &               &     (0.013)   \\	
	
	\hline \hline
	
	\multicolumn{4}{c}{ Dependent Variable: {\bf Log Education Expenditure  } }    \\
	
	
	\hline
	\\
	International Migrant &      -0.492   &               &               \\
Household	&     (0.789)   &               &               \\
	Household Ever had &               &      -0.245   &               \\
International Migrant	&               &     (0.458)   &               \\
	Log Remittances     &               &               &      -0.045   \\
	&               &               &     (0.071)   \\	
	
		\\
	
	
	
	F-statistic	&     266.7361   &    1157.058   &    218.0451   \\
	
	
	\hline \hline
	
	\multicolumn{4}{p{0.60\textwidth}}{\footnotesize Note: All models control for covariates in Table \ref{tab:fullmodel}. The results reported are of IV models instrumented with migration network at Village level and Taluk-Religion level. Clustered standard errors at the village level are reported in the parentheses. The F-statistic refers to the Wald version of the Kleibergen and Paap rk-statistic. The number of observations is 14,325 in all models. * \(p<0.10\), ** \(p<0.05\), *** \(p<0.01\)}
	
\end{longtable}

==> jan 2021/alt_ref.tex <==
\begin{table}[thb!]

	\caption{ Alternative Explanantions - Reference Group Change}\label{tab:alt_ref}
	\begin{tabular}{ >{\arraybackslash}m{1.65in} >{\centering\arraybackslash}m{0.7in} >{\centering\arraybackslash}m{0.7in} >{\centering\arraybackslash}m{0.7in} >{\centering\arraybackslash}m{0.7in}
	>{\centering\arraybackslash}m{0.7in}
	>{\centering\arraybackslash}m{0.7in}	}
		
		\hline\hline
	
	
 	\multicolumn{7}{c}{{Reference Group Income}}    \\

 	\hline 
	    \\          
		
		
		 Migrant Household&       0.408** &       0.443** &       0.443** &       0.404** &       0.471***&       0.513** \\
		 &     (0.160)   &     (0.188)   &     (0.225)   &     (0.164)   &     (0.169)   &     (0.210)   \\
		 
		 \multicolumn{7}{l}{\it Reference Group Income}    \\
		 
		 Mean            &               &      -0.031   &               &               &               &      -0.006   \\
		 &               &     (0.038)   &               &               &               &     (0.049)   \\
		 Median          &               &               &      -0.068   &               &               &      -0.188   \\
		 &               &               &     (0.158)   &               &               &     (0.213)   \\
		 	$90^{th}$ Percentile              &               &               &               &       0.042   &               &       0.109   \\
		 &               &               &               &     (0.071)   &               &     (0.079)   \\
		 Inequality            &               &               &               &               &       0.798** &       0.348   \\
		 &               &               &               &               &     (0.310)   &     (0.362)   \\
		
	 \\
	 
	 F-statistic              &   266.6371   &    113.4875   &    52.37526   &    145.8725   &    169.1362   &    46.26582   \\
	 \\ 
		
		
		
		\hline\hline
		\multicolumn{7}{p{\textwidth}}{\footnotesize Note: Reference group is migrant/non-migrant households in the locality (Taluk). Inequality is calculated as $90^{th} Percentile/25^{th} Percentile$. All models control for covariates in Table \ref{tab:fullmodel}. The results reported are of IV models instrumented with migration network at Village level and Taluk-Religion level. Clustered standard errors at the village level are reported in the parentheses. The F-statistic refers to the Wald version of the Kleibergen and Paap rk-statistic. The number of observations is 14,325 in all models. * \(p<0.10\), ** \(p<0.05\), *** \(p<0.01\) }
		
	\end{tabular}
	
\end{table}

==> jan 2021/balancetable.tex <==

	\begin{table}[tbh!]
		\begin{center}
		\caption{ Difference between Migrant and Non-migrant Households (Key Variables)} \label{tab:balance}
			\begin{tabular}{l*{3}c}
			\hline\hline
			& (1) & (2) & (3) \\
			Variable & Non-migrant & Migrant & Difference \\
			& Household & Household &  \\
			\hline
			\\
			Visible Consumption Index  (PCA)&-0.145&0.676&0.821***\\
			&(1.802)&(1.983)&(0.000)\\
			Visible Consumption Index (Stand.)&-0.070&0.325&0.395***\\
			&(0.976)&(1.045)&(0.000)\\
			Conspicuous Consumption Household &0.320&0.511&0.191***\\
			&(0.467)&(0.500)&(0.000)\\
			Luxury House &0.392&0.609&0.218***\\
			&(0.488)&(0.488)&(0.000)\\
			Household Savings&39,027.941&58,534.859&19,506.918***\\
			&(105751.719)&(133992.438)&(0.000)\\
			Household Investment&79,498.469&124703.430&45,204.965***\\
			&(348990.750)&(427905.094)&(0.000)\\
			Household Debt&138566.641&209846.469&71,279.828***\\
			&(396067.313)&(505044.781)&(0.000)\\
			Food Expenditure&5,648.249&6,646.379&998.130***\\
			&(3,874.706)&(4,037.378)&(0.000)\\
			Education Expenditure&13,805.410&19,767.793&5,962.383***\\
			&(36,786.055)&(46,977.391)&(0.000)\\
			Medical Expenditure &16,396.797&22,905.500&6,508.704***\\
			&(37,576.730)&(47,533.227)&(0.000)\\
			Total Income &21,692.584&28,455.658&6,763.074***\\
			&(26,529.615)&(31,456.730)&(0.000)\\
			Household Size&4.041&4.060&0.020\\
			&(1.684)&(2.007)&(0.637)\\
			Number of Earning Members &1.401&1.908&0.507***\\
			&(0.848)&(0.966)&(0.000)\\
			Male Household Head&0.761&0.509&-0.252***\\
			&(0.427)&(0.500)&(0.000)\\
			Rural Household &0.519&0.515&-0.004\\
			&(0.500)&(0.500)&(0.735)\\
			\hline
			Observations & 12,347 & 2,653 & 15,000 \\
			\hline\hline
			\multicolumn{4}{p{0.86\textwidth}}{\footnotesize Note: Definition of the dependent variables are given in Table \ref{tab:def}. Summary statistics for the entire sample is given in \ref{tab:summary}. Standard Deviations and Standard Errors are reported in the parentheses. * \(p<0.10\), ** \(p<0.05\), *** \(p<0.01\)}
		\end{tabular}
	\end{center}
	\end{table}

	



==> jan 2021/coefgraphs.tex <==
\begin{figure}[thb!]
    \centering
    \caption{ Heterogeneity of Migration Effect - Sub-sample Regressions}
    \begin{subfigure}[t]{0.45 \textwidth}
        \centering
        \includegraphics[width=\linewidth]{incomeclass_s_pca.png} 
        \caption{Income Class} \label{fig:coef1}
    \end{subfigure}
    \hfill
   \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{caste_s_pca.png} 
        \caption{Caste} \label{fig:coef2}
    \end{subfigure}

    \vspace{0.5cm}
    \begin{subfigure}[t]{0.45\textwidth}
    	\centering
    	\includegraphics[width=\linewidth]{religion_s_pca.png} 
    	\caption{Religion} \label{fig:coef3}
    \end{subfigure}
    
	\vspace{0.5cm}
    \caption*{\footnotesize Note:  The results reported are of IV models instrumented with migration network at Village level and Taluk-Religion level. All models control for covariates in Table \ref{tab:fullmodel}. The dependent variable in all regressions is `Visible Consumption Index (PCA)' and the treatment variable is `International Migrant Household'. 95\% confidence interval is plotted along with the coefficient.}
    \label{coef:graph}
\end{figure}
%\newpage

==> jan 2021/coefstab.tex <==
\begin{table}[thb!]
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{ Coefficient Stability Conditions}\label{tab:Costa}
\begin{tabular}{ >{\centering\arraybackslash}m{1.7in} >{\centering\arraybackslash}m{1.2in} >{\centering\arraybackslash}m{1.2in} >{\centering\arraybackslash}m{1.1in} >{\centering\arraybackslash}m{1in}}

\hline\hline
                     
\vspace{3mm}
 %                   &  & (1) & (2) & (3)  (4) \\  
            Dependent Variable        &  Baseline Effect  & Controlled Effect  & Identified Set  & $\delta$ for $\beta = 0$ \\
      &  (Std. Error) $[R^2]$ & (Std. Error) $[R^2]$ & & \\              
\hline 
\\
Visible Consumption       & 0.441***  & 0.228***   & [0.130, 0.414]$^\dag$  &   2.039   \\   
        Index (PCA)         &  (0.029)[0.028] & (0.023)[0.404] & & \\ 
        \\ 

Visible Consumption                & 0.395***   & 0.192*** & [0.099, 0.192]$^\dag$   &   1.870    \\
        Index (Stand.)           &  (0.029)[0.023] & (0.022)[0.406] & & \\   
                     \\ 
                  
Conspicuous Consumption    & 0.191***  & 0.111***  & [ 0.072, 0.111]$^\dag$  &    2.384          \\ 
Household &  (0.129)[0.023] & (0.012)[0.287] & & \\   
\\

Luxury House                    & 0.218***   &  0.145***  & [0.111,  0.145]$^\dag$ &   3.061   \\ 
          &  (0.014)[0.028] & (0.013)[0.244] & & \\   
                                         \\   


\hline\hline
 \multicolumn{5}{p{\textwidth}}{\footnotesize Note: The treatment variable is `International Migrant Household'. Baseline Effect does not include any controls and Controlled Effect has all the control for covariates in Table \ref{tab:fullmodel}. The identified set is bounded by $\hat{\beta}$ of OLS model
 	with controls and $\beta$ calculated given $R_{max} = 1.3 * \tilde{R}$ and $\delta$ = 1. The last column shows
 	the value of $\delta$ which would produce $\beta$ = 0 given the values of $R_{max}$. $\dag$ identified set does not include zero. * \(p<0.10\), ** \(p<0.05\), *** \(p<0.01\)    }

\end{tabular}

\end{table}

==> jan 2021/def.tex <==
\begin{table}[tbh!]
	\caption { Definition of Visible Consumption Indices} \label{tab:def} 
	\begin{tabular}{ >{\arraybackslash}m{6.5 in} }
		\hline \hline
		\vspace{2mm}
		Does the household possess the following? \\
		\vspace{2mm}
		Coding of responses: 0 - No, 1 - Yes  \\
		\vspace{1.5mm}
		(1) Motorcar \\
		(2) Motorcycle \\
		(3) Mobilephone \\
		(4) Television \\
		(5) Refrigerator \\
		(6) Washing Machine \\
		(7) Oven \\
		(8) Computer \\
		(9) Air Conditioner \\
		(10) Inverter \\
		\vspace{1.5mm}	
		{\bf Visible Consumption Index (PCA)} -- Z-score of the Principal Component Analysis value of the above coded responses for 10 goods\\
		\vspace{1.5mm}
		{\bf Visible Consumption Index (Standarized)} -- After taking standardized value for each of these ten goods, a sum total of these ten standardized scores is taken for each household, which is again standardized\\
		\vspace{1.5mm}
		{\bf Conspicuous Consumption Household (Least Possessed)} -- Household possesses at least one of the five least possessed goods in the region (Taluk)\\
		\\
		\midrule
		\\
		Type of house which the household is now occupying\\
		\vspace{2mm}
		Coding of responses: \\
		1 - Luxurious (3 or more bedrooms with attached bathrooms, concrete/tile roof, tiled
		floor) \\
		2 - Very Good (2 bed rooms with attached bathrooms, concrete/tile roof, Mosaic
		floor) \\
		3 - Good (1 bed room, brick and cement walls, concrete or tile roof) \\
		4 - Poor
		(Brick walls, cement floor, tin or asbestos roof) \\
		5 - Kutcha (Mud walls, Mud floor \& Thatched roof) \\
		\vspace{1.5mm}	
		{\bf Luxury House} -- Response 1 or 2\\
		\\
		\hline \hline
		\end {tabular}
\end{table}

==> jan 2021/financials.tex <==
\begin{longtable}[t]{l c c c }
	
	
	\caption{IV Results for the Effect of
		Migration on Household Financials \label{tab:reg_fin}} \\
	%
	
	\hline \hline
	\endfirsthead
	
	\multicolumn{4}{l}%
	{{ \tablename\ \thetable{} -- continued from previous page}} \\
	\hline
	\endhead
	
	\hline
	\multicolumn{4}{r}{{Continued on next page}} \\
	\endfoot	
	
	\endlastfoot
	
	
	
	\multicolumn{4}{c}{{ Dependent Variable: {\bf Log Savings} }}    \\
	\hline
	International Migrant 		&  1.520      &              &               \\
	Household	&   (1.505)     &              &            \\		
	\\
	Household Ever had  	&        &      0.603        &              \\
	International Migrant	&        &       (0.876)       &           \\
	\\	
	Log Remittances	&        &               &        0.142     \\
	&        &               &       (0.135)     \\	
	
	\hline \hline
	
	\multicolumn{4}{c}{{ Dependent Variable: {\bf Log Investment} }}    \\
	\hline
	International Migrant 		& -4.541***      &              &               \\
	Household	&    (1.662)     &              &            \\		
	\\
	Household Ever had  	&        &      -2.657***        &              \\
	International Migrant	&        &        (0.984)       &           \\
	\\	
	Log Remittances	&        &               &       -0.406***     \\
	&        &               &       (0.149)    \\		
	\hline \hline
	
	
	\multicolumn{4}{c}{{ Dependent Variable: {\bf Log Debt} }}    \\
	\hline
	International Migrant 		&  2.777*      &              &               \\
	Household	&   (1.571)     &              &            \\		
	\\
	Household Ever had  	&        &      1.862**        &              \\
	International Migrant	&        &       (0.908)       &           \\
	\\	
	Log Remittances	&        &               &         0.242*     \\
	&        &               &       (0.140)     \\	
	
	\\
	
	F-statistic	&               266.637      &           1159.263 &     218.153  \\
	
	
	\hline \hline
	
	\multicolumn{4}{p{0.60\textwidth}}{\footnotesize Note: All models control for covariates in Table \ref{tab:fullmodel}. The results reported are of IV models instrumented with migration network at Village level and Taluk-Religion level. Clustered standard errors at the village level are reported in the parentheses. The F-statistic refers to the Wald version of the Kleibergen and Paap rk-statistic. The number of observations is 14,325 in all models. * \(p<0.10\), ** \(p<0.05\), *** \(p<0.01\)}
	
\end{longtable}

==> jan 2021/fullcontrol.tex <==
\begin{longtable}[thb!]{l  c  c c }
	\caption{ OLS Results -- Visible Consumption Index (PCA) -- Full Controls \label{tab:fullmodel}} \\
%

\hline \hline
 & (1) & (2) & (3)\\
\hline \endfirsthead

\multicolumn{4}{l}%
{{ \tablename\ \thetable{} -- continued from previous page}} \\
\hline
&\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
\hline 
\endhead

\hline \multicolumn{4}{r}{{Continued on next page}} \\
\endfoot	

\endlastfoot


		\\
		International Migrant Household&       0.228***&               &               \\
	   &     (0.023)   &               &               \\
		Household Ever had International Migrant&              &       0.222***&               \\
		&               &       (0.019)   &               \\
		Log Remittances   &              &               &       0.019***\\
		&               &               &      (0.002)   \\
		Household Income       &  0.051***&       0.051***&       0.050***\\
		&     (0.006)   &     (0.006)   &     (0.006)   \\
		
		Religion \\
		{\it (Reference - Hindu)}             &                &                &                \\
		\hspace{5mm} Christian   &     0.191***&       0.189***&       0.193***\\
		&     (0.024)   &     (0.024)   &     (0.024)   \\
		\hspace{5mm} Muslim  &  0.215***&       0.199***&       0.219***\\
		&     (0.025)   &     (0.026)   &     (0.025)   \\
		Highest Education in the Household\\
		{\it (Reference - School or less)}             &                &                &                \\
		\hspace{5mm}Higher Secondary    &    0.181***&       0.180***&       0.183***\\
		&     (0.016)   &     (0.016)   &     (0.016)   \\
		\hspace{5mm} College    &      0.385***&       0.389***&       0.387***\\
		&     (0.019)   &     (0.019)   &     (0.019)   \\
		\hspace{5mm} Other Higher Education    &   0.772***&       0.774***&       0.779***\\
		&     (0.028)   &     (0.027)   &     (0.027)   \\
		Rural Household     &     -0.170***&      -0.165***&      -0.169***\\
		&     (0.026)   &     (0.027)   &     (0.026)   \\
		Male Household Head &       0.037***&       0.021   &       0.038***\\
		&     (0.014)   &     (0.014)   &     (0.014)   \\
		Number of earning individuals in the HH&        -0.013   &      -0.009   &      -0.009   \\
		&     (0.009)   &     (0.009)   &     (0.009)   \\
		Household Size              &      0.008*  &       0.003   &       0.006   \\
		&     (0.005)   &     (0.005)   &     (0.005)   \\
		Type of Ration Card\\
		{\it (Reference - BPL)}\\
		\hspace{5mm}      APL          &     0.390***&       0.389***&       0.390***\\
		&     (0.016)   &     (0.016)   &     (0.016)   \\
		\hspace{5mm} Non-priority              &      1.009***&       1.013***&       1.011***\\
		&     (0.026)   &     (0.026)   &     (0.026)   \\
		\\	
		District Dummies & Yes & Yes & Yes \\
		
		\hline
		R-squared           &    .404   &     .406   &    .404   \\
		No. of Observations &       14325   &       14325   &       14325   \\
	%	R-squared           &    .404   &     .406   &    .404   \\
		\hline\hline
		\multicolumn{4}{p{0.80\textwidth}}{\footnotesize Note: Standard errors clustered at the village level are reported in the parentheses. * \(p<0.10\), ** \(p<0.05\), *** \(p<0.01\)}\\
\end{longtable}


==> jan 2021/overtime.tex <==
	\begin{table}[tbh!]
	\begin{center}
		\caption{ Pooled Cross-sectional Data Analysis} \label{tab:overtime}
		
		\begin{tabular}{l*{2}{c}}
			\hline\hline
			&\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
			
			
			Migrant Household&       0.441***&       0.732** \\
			&     (0.138)   &     (0.324)   \\
			2018  Round             &      -0.080***&       0.007   \\
			&     (0.024)   &     (0.066)   \\
			2016  Round            &       0.078***&       0.155** \\
			&     (0.026)   &     (0.061)   \\
			Migrant HH * 2018       &               &      -0.436   \\
			&               &     (0.295)   \\
			Migrant HH * 2016       &               &      -0.417   \\
			&               &     (0.300)   \\
			\\
			F-statistic                   &      573.372         &      65.220         \\
			\hline\hline
			\multicolumn{3}{p{0.6\textwidth}}{\footnotesize Note: The results reported are of IV models instrumented with migration network at Village level and Taluk-Religion level. The dependent variable in all regressions is `Visible Consumption Index (PCA)' and the treatment variable is `International Migrant Household'. All models control for covariates in Table \ref{tab:fullmodel}. Clustered standard errors at the village level are reported in the parentheses. The F-statistic refers to the Wald version of the Kleibergen and Paap rk-statistic. The number of observations is 41,782 in all models. * \(p<0.10\), ** \(p<0.05\), *** \(p<0.01\)}\\
		\end{tabular}
	
\end{center}
\end{table}


==> jan 2021/pcs.tex <==
\begin{longtable}[thb!]{l c c c c c c}
	
	
	\caption{Regression Results for the Effect of
		Migration on Visible Consumption Index (PCA) \label{tab:reg_pca}} \\
	%
	
	\hline \hline
	\endfirsthead
	
	\multicolumn{7}{l}%
	{{ \tablename\ \thetable{} -- continued from previous page}} \\
	\hline
	\endhead
	
	\hline
	\multicolumn{7}{r}{{Continued on next page}} \\
	\endfoot	
	
	\endlastfoot
	
	

	
	&  \underline{OLS}   &    \underline{IV-2SLS}      &    \underline{OLS}   &    \underline{IV-2SLS} &  \underline{OLS}   &    \underline{IV-2SLS}  \\
	\\
	International Migrant 		&      0.228***&       0.408** &               &               &               &               \\
	Household	&    (0.023)   &     (0.160)   &               &               &               &               \\
	\\
	Household Ever had  	&              &               &       0.222***&       0.240***&               &               \\
	International Migrant	&              &               &     (0.019)   &     (0.093)   &               &               \\
	\\	
	Log Remittances	&                   &               &               &               &       0.019***&       0.036** \\
	&               &               &               &               &     (0.002)   &     (0.014)   \\	
		
	\\
	
	F-statistic	&      &         266.637      &      &     1159.263 &  &   218.153  \\
	\hline \hline
	
	\multicolumn{7}{p{0.86\textwidth}}{\footnotesize Note: Definition of the dependent variables are given in Table \ref{tab:def}. All models control for covariates in Table \ref{tab:fullmodel}. IV models are instrumented with migration network at Village level and Taluk-Religion level. Clustered standard errors at the village level are reported in the parentheses. The F-statistic refers to the Wald version of the Kleibergen and Paap rk-statistic. The number of observations is 14,325 in all models. * \(p<0.10\), ** \(p<0.05\), *** \(p<0.01\)}
	
\end{longtable}

==> jan 2021/summstat.tex <==
\begin{longtable}[thb!]{ l c c c c}
	\caption { Summary Statistics} \label{tab:summary} \\
		

\hline \hline
\multicolumn{1}{l}{\textbf{Variable}} & \multicolumn{1}{c}{\textbf{Mean (Proportion)}} & \multicolumn{1}{c}{\textbf{Std. Deviation}}  & \multicolumn{1}{c}{\textbf{Min}} & \multicolumn{1}{c}{\textbf{Max}}\\ \hline 
\endfirsthead
		
\multicolumn{5}{l}%
{{ \tablename\ \thetable{} -- continued from previous page}} \\
\hline \multicolumn{1}{l}{\textbf{Variable}} & \multicolumn{1}{c}{\textbf{Mean (Proportion)}} & \multicolumn{1}{c}{\textbf{Std. Deviation}}  & \multicolumn{1}{c}{\textbf{Min}} & \multicolumn{1}{c}{\textbf{Max}}\\ \hline
\endhead

\hline \multicolumn{5}{r}{{Continued on next page}} \\
\endfoot	
			
\hline \hline
\endlastfoot
		\\
		\textit{Dependent variables}\\
\\
		Visible Consumption Index  (PCA)  &  0.00 &	1.86	& -2.60	& 5.52  \\
	
			Visible Consumption Index (Stand.)   &  0.00 &	1.00	& -1.97	& 2.88  \\
	Conspicuous Consumption Household     &  0.35 &	-   &	- &	- \\
		Luxury House & 0.43 &	-   &	- &	-\\
		
		
		Household Savings &  42477 &	111513   &	0 & 1098500\\
		Household Investment &  87493 &	364587   &	0 &	4500000\\
		Household Debt &  151173 &	418284   &	0 &	4500000\\
		
		
		Food Expenditure &  5824 &	3922   &	400 & 40000\\
		Education Expenditure &  14859 &	38848   &	0 &	400000\\
		Health Expenditure &  17547 &	39597   &	0 &	416000\\
		\\
		
		
		\textit{Instrument variables}\\
		\\
		Migration Network (Village Level) & 0.28 & 0.20 & 0.00 & 0.93 \\
		Migration Network  & 0.28 & 0.20 & 0.00 & 1.00 \\
		(Same Religion at Taluk Level)	& & & & \\
		\\
		
		\textit{Treatment variables}\\
		\\
		Household with International Migrant & 0.18 &	-   &	- &	-\\
		Household ever had International Migrant & 0.28 &	-   &	- &	-\\
		Remittances & 185641 &  171337 &0 & 802500 \\
		\\
		
		\textit{Control variables}\\
		\\
		Household Income & 22888 &  27585 &  0 &  300000\\
		Household Size & 4.04 &  1.75& 1& 18\\
		Number of Earning Members &  1.49 &  0.89 & 0 & 8\\
		Male Household Head & 0.72 &	-   &	- &	-\\
		Rural Household & 0.52 &	-   &	- &	-\\
		
	
		Religion \\
		\hspace{6mm}		Hindu & 0.56 &	-   &	- &	-\\
		\hspace{6mm}		Muslim & 0.23 &	-   &	- &	-\\
		\hspace{6mm}		Christian  & 0.21 &	-   &	- &	-\\
		Highest education in the household \\
		\hspace{6mm}	School or less & 0.26 &	-   &	- &	-\\
		\hspace{6mm}	Higher Secondary  & 0.29 &	-   &	- &	-\\
		\hspace{6mm}	College  & 0.24 &	-   &	- &	-\\
		\hspace{6mm}	Other Higher Education & 0.21 &	-   &	- &	-\\
		Type of Ration Card \\
		\hspace{6mm}	BPL & 0.39 &	-   &	- &	-\\
		\hspace{6mm}	APL & 0.40 &	-   &	- &	-\\
		\hspace{6mm}	 Non-priority   & 0.21 &	-   &	- &	-\\
		
		

		\end{longtable}
